The 26 Wilf-equivalence classes of length five quasi-consecutive patterns

We present two families of Wilf-equivalences for consecutive and quasi-consecutive vincular patterns. These give new proofs of the classification of consecutive patterns of length $4$ and $5$. We then prove additional equivalences to explicitly classify all quasi-consecutive patterns of length $5$ into 26 Wilf-equivalence classes.

==> biject.tex <==
\section{A family of bijective equivalences}
\label{sec:BijectionCons}

In the result, we prove a family of Wilf-equivalences for
consecutive and quasi-consecutive patterns.
This will give new proofs of all consecutive Wilf-equivalences of length $4$ and $5$.

\begin{theorem} \label{thm:BijectionCons}
    Suppose that 
	\[ \sigma = \sigma_1\sigma_2\cdots\sigma_i\sigma_{i+1}\cdots
		\sigma_{j}\sigma_{j+1}\cdots\sigma_k \]
	is a permutation where $1 \le i < j < k.$ 
	Also suppose that 
	\[ \tau = \tau_1\tau_2\cdots\tau_i\tau_{i+1}\cdots
		\tau_j\tau_{j+1}\cdots\tau_k \]
	where $\tau_{i+1}, \dots, \tau_j$ is a permutation of
	$\sigma_{i+1}, \dots, \sigma_j$, and $\sigma_x = \tau_x$
	for $x \in [1,i] \cup [j+1, k]$.
	Finally, suppose that
	\begin{align*}
		\sigma_1\cdots\sigma_z &\not\sim \sigma_{k-z+1}\cdots\sigma_k \\
		\sigma_1\cdots\sigma_z &\not\sim \tau_{k-z+1}\cdots\tau_k \\
		\sigma_1'\cdots\sigma_z' &\not\sim \sigma_{k-z+1}\cdots\sigma_k \\
		\sigma_1'\cdots\sigma_z' &\not\sim \tau_{k-z+1}\cdots\tau_k
	\end{align*}
	all hold for $z > \min(i, k-j)$, $z \neq  k$.
	Then, \[ \sigma \equiv \tau. \]
\end{theorem}

\begin{proof}
    We present a bijection mapping permutations of $S_n$ containing $\sigma$ (call the set $T_n$) to permutations of $S_n$ containing $\tau$ (call the set $T_n'$.)  Note $T_n$ and $T_n'$ need not be disjoint. For each such permutation in $T_n \cup T_n'$, draw a box of length $k$ around every occurrence of $\sigma$ or $\tau$.  Because of the four equivalences not occurring, no two boxes can intersect in more than $\min(i, k-j)$ places.  Also since $i < j$ we cannot have three boxes pairwise intersecting.
    
    Consider the following map $\Psi$ from $T_n \cup T_n'$ to itself by permuting every boxed $\sigma$ permutation to make it a $\sigma'$ permutation and vice versa.  Because boxes do not intersect in more than $\min(i, k-j)$ places, the order of permutation does not matter.  This also means that $\Psi$ sends $T_n$ to $T_n'$ and $T_n'$ to $T_n,$ showing us that $\Psi$ is a well defined map.
    
    Also, our four equivalence restrictions prevent new $\sigma$ or $\tau$ permutations from appearing because a new occurrence of $\sigma$ or $\tau$ would need to have at least one element in a block of $k$ elements changed.  Thus, it would need to intersect with a part of a boxed segment in at least one of positions $i+1, ..., j$, a clear contradiction.  Now, note that for $\pi \in T_n \cup T_n'$ the boxes around $\pi$ will be the same as the boxes around $\Psi(\pi).$  This means that $\Psi \circ \Psi$ is the identity map, because every box will permute from $\sigma$ to $\tau$ to $\sigma$ again, or vice versa.  Thus, we have a bijection from $T_n$ to $T_n'$ given by $\Psi,$ so we are done.
\end{proof}

\begin{corollary}
	\label{cor:known45}
    The following equivalences hold:
	\begin{itemize}
		\item $1342 \equiv 1432$
		\item $13452 \equiv 13542 \equiv 14352 \equiv 14532 \equiv 15342 \equiv 15432$
		\item $12453 \equiv 12543$
		\item $24153 \equiv 25143$.
	\end{itemize}
\end{corollary}

The first equivalence in fact represents all Wilf-equivalences
of consecutive patterns of length 4,
and the next three equivalences represent all Wilf-equivalences
of consecutive patterns of length 5.
Thus, our theorem provides a simple bijective proof of the
consecutive cases for length 4 and 5 patterns.
Our theorem is not sufficient for length 6 patterns.

We can extend Theorem \ref{thm:BijectionCons} to
permutations of the form $\sigma_1 \cdots \sigma_k \text{-} \sigma_{k+1}$.

\begin{theorem}  \label{thm:BijectionVinc}
    Suppose that 
	\[ \sigma = \sigma_1\sigma_2\cdots\sigma_i
		\sigma_{i+1}\cdots\sigma_{j}
		\sigma_{j+1}\cdots\sigma_k \]
	is a permutation where $1 \le i < j < k$.
	Also suppose that 
	\[ \sigma' = \sigma_1'\sigma_2'\cdots\sigma_i\sigma_{i+1}'\cdots
		\sigma_{j}'\sigma_{j+1}'\cdots\sigma_k' \]
	where $\sigma_{i+1}',\dots,\sigma_{j}'$ is a permutation of $\sigma_{i+1}, \dots, \sigma_j$,
	and $\sigma_x = \sigma_x'$ for $1 \le x \le i, j+1 \le x \le n$.
	Finally, suppose that
	\begin{align*}
		\sigma_1\cdots\sigma_z &\not\sim \sigma_{k-z+1}\cdots\sigma_k \\
		\sigma_1\cdots\sigma_z &\not\sim \sigma_{k-z+1}'\cdots\sigma_k' \\
		\sigma_1'\cdots\sigma_z' &\not\sim \sigma_{k-z+1}\cdots\sigma_k \\
		\sigma_1'\cdots\sigma_z' &\not\sim \sigma_{k-z+1}'\cdots\sigma_k'
	\end{align*}
	all hold for $z > \min(i, k-j)$, $z \neq  k$.
	Then, \[ \sigma \equiv \tau. \]
\end{theorem}

\begin{proof}
    The argument is quite similar to that given in Theorem \ref{thm:BijectionCons}.  Again, consider the sets $T_n \subset S_n$ containing $\sigma_1\cdots\sigma_k$ permutations, $T_n' \subset S_n$ containing $\tau_1\cdots\tau_k$ and a map $\Psi$ from $T_n \cup T_n'$ to itself in the same way.  We show that $\Psi$ bijects elements in $T$ containing $\sigma$ to elements in $T'$ containing $\tau.$
    
    To see why, suppose that $\pi$ in $T$ contains $\sigma$.  Specifically, say that $\pi_t\pi_{t+1}\cdots\pi_{t+k-1} \pi_z \sim \sigma_1\cdots\sigma_{k+1}$ where $1 \le t, t+k \le z \le n.$  Then, $\Psi$ sends $\pi_t\pi_{t+1}\cdots\pi_{t+k-1}$ to a permutation which is order isomorphic to $\tau_1\cdots\tau_k$, and either $\pi_z$  maps to itself or the value corresponding to $\pi_z$ would move to a position still after position $t+k-1,$ meaning that $\tau$ is still there.  Thus, we are done.
\end{proof}

\begin{corollary} \label{cor:Bijective5quasi}
    The following equivalences hold:
	\begin{enumerate}
		\item[(A2)] $1453\-2 \equiv 1543\-2$
		\item[(E2)] $3125\-4 \equiv 3215\-4$.
	\end{enumerate}
\end{corollary}



